Investigating Lane-Free Traffic with a Dynamic Driving Simulator

Lane-free traffic (LFT) is a new traffic system that relies on connected and automated vehicles (CAV) to increase road capacity and utilization by removing traditional lane markings using coordinated maneuvering of CAVs in LFT strategies. LFT is based on two main principles: upstream nudging and vehicles moving without adhering to any lane markings. By leveraging CAV capabilities to communicate and exchange information, LFT represents a promising future traffic system. While current research uses LFT simulations in two-dimensional space, driving simulators are necessary to investigate human behavior and perceived safety in LFT. This paper proposes a conceptual framework for LFT driving simulations and describes the assumptions, requirements, and recent technological developments that make it possible to investigate the human perspective and acceptance of LFT. Additionally, we propose a scenario matrix that can act as a test guide to building driving simulation scenarios for the LFT.

==> Bibliography/Laneless <==
{\rtf \tx504 \li504 \fi-504 \sl240 \slmult1 \sa0 [1]\tab \uc0\u8216{}Journal of the Eastern Asia Society for Transportation Studies\uc0\u8217{}, p. 15.
\
[2]\tab \uc0\u8216{}Archives of Transport\uc0\u8217{}, {\i{}Archives of Transport}, p. 14, 2018.
\
[3]\tab \uc0\u8216{}Asian Transport Studies, Volume 4, Issue 2 (2016), 379\uc0\u8211{}391\uc0\u8217{}, vol. 4, no. 2, p. 13, 2016.
\
[4]\tab H. Xie, J. Zhu, and H. Duan, \uc0\u8216{}Analysis of the Relationship between the Density and Lane-Changing Behavior of Circular Multilane Urban Expressway in Mixed Traffic\uc0\u8217{}, {\i{}Journal of Advanced Transportation}, vol. 2022, pp. 1\uc0\u8211{}40, Jan. 2022, doi: 10.1155/2022/4499477.
\
[5]\tab S. Srikanth, A. Mehar, and K. G. N. V. Praveen, \uc0\u8216{}Simulation of Traffic Flow to Analyze Lane Changes on Multi-lane Highways under Non-lane Discipline\uc0\u8217{}, {\i{}Period. Polytech. Transp. Eng.}, vol. 48, no. 2, pp. 109\uc0\u8211{}116, Jan. 2018, doi: 10.3311/PPtr.10150.
\
[6]\tab D. S. M. Santhakumar, \uc0\u8216{}Driving Behavior and Safety Analysis In Context Of Weak Lane Discipline At Urban Mid-Block Section\uc0\u8217{}, p. 13, 2021.
\
[7]\tab P. Saha, A. K. Sarkar, and M. Pal, \uc0\u8216{}EVALUATION OF SPEED\uc0\u8211{}FLOW CHARACTERISTICS ON TWO-LANE HIGHWAYS WITH MIXED TRAFFIC\uc0\u8217{}, {\i{}TRANSPORT}, vol. 32, no. 4, pp. 331\uc0\u8211{}339, Jan. 2015, doi: 10.3846/16484142.2015.1004369.
\
[8]\tab V. Papathanasopoulou and C. Antoniou, \uc0\u8216{}Towards an integrated longitudinal and lateral movement data-driven model for mixed traffic\uc0\u8217{}, {\i{}Transportation Research Procedia}, vol. 37, pp. 489\uc0\u8211{}496, 2019, doi: 10.1016/j.trpro.2018.12.214.
\
[9]\tab D. Pal, S. P. Venthuruthiyil, and M. Chunchu, \uc0\u8216{}Characteristics of Vehicular Lateral Shifts in Non-lane-disciplined Traffic Stream\uc0\u8217{}, {\i{}Transportation Research Procedia}, vol. 48, pp. 3245\uc0\u8211{}3253, 2020, doi: 10.1016/j.trpro.2020.08.153.
\
[10]\tab A. Nagahama, T. Wada, D. Yanagisawa, and K. Nishinari, \uc0\u8216{}Detection of leader\uc0\u8211{}follower combinations frequently observed in mixed traffic with weak lane-discipline\uc0\u8217{}, {\i{}Physica A: Statistical Mechanics and its Applications}, vol. 570, p. 125789, May 2021, doi: 10.1016/j.physa.2021.125789.
\
[11]\tab M. Mushfiq {\i{}et al.}, \uc0\u8216{}To Lane or Not to Lane? Comparing On-Road Experiences in Developing and Developed Countries using a New Simulator \uc0\u8220{}RoadBird\uc0\u8221{}\uc0\u8217{}, p. 22.
\
[12]\tab C. R. Munigety, \uc0\u8216{}Modelling behavioural interactions of drivers\uc0\u8217{} in mixed traffic conditions\uc0\u8217{}, {\i{}Journal of Traffic and Transportation Engineering (English Edition)}, vol. 5, no. 4, pp. 284\uc0\u8211{}295, Aug. 2018, doi: 10.1016/j.jtte.2017.12.002.
\
[13]\tab A. K. Mulla, A. Joshi, R. Chavan, D. Chakraborty, and D. Manjunath, \uc0\u8216{}A Microscopic Model for Lane-Less Traffic\uc0\u8217{}, {\i{}IEEE Trans. Control Netw. Syst.}, vol. 6, no. 1, pp. 415\uc0\u8211{}428, Mar. 2019, doi: 10.1109/TCNS.2018.2834313.
\
[14]\tab Ch. Mallikarjuna and K. R. Rao, \uc0\u8216{}AREA OCCUPANCY CHARACTERISTICS OF HETEROGENEOUS TRAFFIC\uc0\u8217{}, {\i{}Transportmetrica}, vol. 2, no. 3, pp. 223\uc0\u8211{}236, Jan. 2006, doi: 10.1080/18128600608685661.
\
[15]\tab G. Mahapatra and A. K. Maurya, \uc0\u8216{}Dynamic parameters of vehicles under heterogeneous traffic stream with non-lane discipline: An experimental study\uc0\u8217{}, {\i{}Journal of Traffic and Transportation Engineering (English Edition)}, vol. 5, no. 5, pp. 386\uc0\u8211{}405, Oct. 2018, doi: 10.1016/j.jtte.2018.01.003.
\
[16]\tab G. Mahapatra and A. K. Maurya, \uc0\u8216{}Study of Vehicles Lateral Movement in Non-lane Discipline Traffic Stream on a Straight Road\uc0\u8217{}, {\i{}Procedia - Social and Behavioral Sciences}, vol. 104, pp. 352\uc0\u8211{}359, Dec. 2013, doi: 10.1016/j.sbspro.2013.11.128.
\
[17]\tab K. Madhu, R. Sivanandan, and K. K. Srinivasan, \uc0\u8216{}Identification of different vehicle-following manoeuvres for heterogeneous weak-lane disciplined traffic condition from vehicle trajectory data\uc0\u8217{}, {\i{}IOP Conf. Ser.: Earth Environ. Sci.}, vol. 491, no. 1, p. 012052, Jun. 2020, doi: 10.1088/1755-1315/491/1/012052.
\
[18]\tab S. K. M. and A. Verma, \uc0\u8216{}Review of Studies on Mixed Traffic Flow: Perspective of Developing Economies\uc0\u8217{}, {\i{}Transp. in Dev. Econ.}, vol. 2, no. 1, p. 5, Apr. 2016, doi: 10.1007/s40890-016-0010-0.
\
[19]\tab V. Kanagaraj, G. Asaithambi, T. Toledo, and T.-C. Lee, \uc0\u8216{}Trajectory Data and Flow Characteristics of Mixed Traffic\uc0\u8217{}, {\i{}Transportation Research Record}, vol. 2491, no. 1, pp. 1\uc0\u8211{}11, Jan. 2015, doi: 10.3141/2491-01.
\
[20]\tab H. Farah, A. Polus, S. Bekhor, and T. Toledo, \uc0\u8216{}Study of passing gap acceptance behavior using a driving simulator\uc0\u8217{}, p. 9, 2007.
\
[21]\tab A. Dhamaniya and S. Chandra, \uc0\u8216{}Speed Characteristics of Mixed Traffic Flow on Urban Arterials\uc0\u8217{}, {\i{}International Journal of Civil and Environmental Engineering}, vol. 7, no. 11, p. 6, 2013.
\
[22]\tab A. K. Budhkar and A. K. Maurya, \uc0\u8216{}Characteristics of lateral vehicular interactions in heterogeneous traffic with weak lane discipline\uc0\u8217{}, {\i{}J. Mod. Transport.}, vol. 25, no. 2, pp. 74\uc0\u8211{}89, Jun. 2017, doi: 10.1007/s40534-017-0130-1.
\
[23]\tab G. Babu and S. Biradar, \uc0\u8216{}Study and Analysis of Road Widening and Strengthening\uc0\u8217{}, p. 9, 2021.
\
[24]\tab G. Asaithambi, V. Kanagaraj, and T. Toledo, \uc0\u8216{}Driving Behaviors: Models and Challenges for Non-Lane Based Mixed Traffic\uc0\u8217{}, {\i{}Transp. in Dev. Econ.}, vol. 2, no. 2, p. 19, Oct. 2016, doi: 10.1007/s40890-016-0025-6.
\
[25]\tab G. Asaithambi, V. Kanagaraj, and T. Toledo, \uc0\u8216{}Driving Behaviors: Models and Challenges for Non-Lane Based Mixed Traffic\uc0\u8217{}, {\i{}Transp. in Dev. Econ.}, vol. 2, no. 2, p. 19, Oct. 2016, doi: 10.1007/s40890-016-0025-6.
\
[26]\tab M. Agrawal and K. Vemuri, \uc0\u8216{}SIMULATING AND ANALYZING CHAOS OF INDIAN TRAFFIC CONDITION\uc0\u8217{}, p. 9.
\
[27]\tab \uc0\u8216{}Paper-QuantitativedeterminationofVehicleInfluence.pdf\uc0\u8217{}.
 \
[28]\tab \uc0\u8216{}Notes.txt\uc0\u8217{}.
 \
[29]\tab \uc0\u8216{}Flexible car-following models for mixed traffic and weak lane-discipline conditions _ Enhanced Reader.pdf\uc0\u8217{}.
 \
}
